GaussianAnything: Interactive Point Cloud Flow Matching For 3D Object Generation

While 3D content generation has advanced significantly, existing methods still face challenges with input formats, latent space design, and output representations. This paper introduces a novel 3D generation framework that addresses these challenges, offering scalable, high-quality 3D generation with an interactive Point Cloud-structured Latent space. Our framework employs a Variational Autoencoder (VAE) with multi-view posed RGB-D(epth)-N(ormal) renderings as input, using a unique latent space design that preserves 3D shape information, and incorporates a cascaded latent flow-based model for improved shape-texture disentanglement. The proposed method, GaussianAnything, supports multi-modal conditional 3D generation, allowing for point cloud, caption, and single image inputs. Notably, the newly proposed latent space naturally enables geometry-texture disentanglement, thus allowing 3D-aware editing. Experimental results demonstrate the effectiveness of our approach on multiple datasets, outperforming existing native 3D methods in both text- and image-conditioned 3D generation.

==> sections/discussions.tex <==
\subsection{Limitations and future work}

Limitations:
The 3D shapes of the objects discussed in this paper can still be encoded with a single latent code.

% A similar observation is also found in~\cite{esser2024sd3}, where separate model parameters handle different modalities individually. 

Future work:
geometry side:
3D shapes with large variations such as human.
more complex, adopt local features to predict the geometry along with the global features.

texture side:
currently we only adopt a basic 2D hour-glass encoder to restoring the missing 3D information form the naive GAN inversion,
a more geometry-aware architecture such as 3D convolution used in cost volume based reconstruction methods~\misscite would likely to further improve the reconstruction performance on the novel views.

training side:
currently we need an extra 2D alignment module to assist the editing though lite, still introduces extra computational cost.
In the future work, we aim to find ways to remove this module without sacrificing the reconstruction ability,
and propose an end-to-end training strategy.

Overall,
we believe this work opens a new line of research direction and could serve as a guidance for future works beyond 3D GAN inversion, 
also few-shot 3D reconstructions and 3D-aware learning from 2D images, etc. 

\yslan{contribute: the merits of both priors.}

\yslan{out method could be easily extended to multi-view input.}


and takes a step towards expected 3D GAN inversion.


\heading{Limitations}
disadvantages:
slow sampling.

==> tables/abla-gaussian-utilization-ratio.tex <==

\begin{table}[h!]
% \vspace{-6mm}
\centering
% \hfill % !
% \begin{minipage}[b]{0.48\textwidth}
    \centering
    \caption{\textbf{Gaussian Utilization Ratio.} 
    \yslan{shrink the margin.} 
    We compare the effective Gaussians (opacity $>0.005$) used during splatting here. Pixel-aligned Gaussian prediction methods waste a large portion of Gaussians when representing 3D object, while our proposed framework yields more compact results.}
    \begin{tabular}{lc}
        \toprule
        Method & Effective GS ($\%$)  \\
        \midrule
        Splatter Image & {17.14} \\
        LGM & {52.63} \\
        Ours & \textbf{96.84} \\
        \bottomrule
    \end{tabular}
    \label{tab:abla:gaussian-utilization}%
% \end{table}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.49\textwidth}
%    \centering 
%     \captionof{table}{\textbf{Diffusion Sampling Speed and Latent Size}. We provide the sampling time per instance evaluated on $1$ V100, along with the latent size. 
%     Our method achieves faster sampling speed while maintaining superior generation performance.
%     }
%     \begin{tabular}{lcc}
%         \toprule
%         Method & V100-sec &  Latent Size \\
%         \midrule
%         Get3D/EG3D &{<0.5} & 256 \\
%         \midrule
%         SSDNeRF &{8.1} & $128^2\times18$ \\
%         RenderDiffusion & {15.8} & - \\
%         DiffRF & {18.7} & $32^3 \times 4$ \\
%         \nickname{}$_\text{uncond}$ &\textbf{5.7} &  $32^2\times12$ \\
%         \nickname{}$_\text{cfg}$ & \textbf{7.5} & $32^2\times12$ \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:exp:sampling_speed_and_latent_size}%
% \end{minipage}
% \vspace{-4mm}
\end{table}

==> tables/abla-table.tex <==
\begin{table}[h!]
% \vspace{-6mm}
\centering
% \hfill % !
% \begin{minipage}[b]{0.48\textwidth}
    \centering
    % \captionof{table}{\textbf{Ablation of 3D VAE Design.} We ablate the design of our auto-encoding architecture. Each component contributes to a consistent gain in the reconstruction performance, indicating an improvement in the modeling capacity.}
    \caption{\textbf{Ablation of 3D VAE Design.} 
    \yslan{shrink the margin.} 
    We ablate the design of our 3D VAE architecture. Each component contributes to a consistent gain in the reconstruction performance, indicating an improvement in the modeling capacity.}
    \begin{tabular}{lc}
        \toprule
        Design & LPIPS@100K  \\
        \midrule
        Dense Point Cloud as Input & {0.174} \\
        \midrule
        Multi-view RGB-D as Input &{0.163} \\
        + Normal Map &{0.157} \\
        + Gaussian Upsampling Module &{0.095} \\
        + 3 $\times$ Gaussian Upsampling Module & \textbf{0.067} \\
        \bottomrule
    \end{tabular}
    \label{tab:abla:rec_arch}%
% \end{table}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.49\textwidth}
%    \centering 
%     \captionof{table}{\textbf{Diffusion Sampling Speed and Latent Size}. We provide the sampling time per instance evaluated on $1$ V100, along with the latent size. 
%     Our method achieves faster sampling speed while maintaining superior generation performance.
%     }
%     \begin{tabular}{lcc}
%         \toprule
%         Method & V100-sec &  Latent Size \\
%         \midrule
%         Get3D/EG3D &{<0.5} & 256 \\
%         \midrule
%         SSDNeRF &{8.1} & $128^2\times18$ \\
%         RenderDiffusion & {15.8} & - \\
%         DiffRF & {18.7} & $32^3 \times 4$ \\
%         \nickname{}$_\text{uncond}$ &\textbf{5.7} &  $32^2\times12$ \\
%         \nickname{}$_\text{cfg}$ & \textbf{7.5} & $32^2\times12$ \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:exp:sampling_speed_and_latent_size}%
% \end{minipage}
% \vspace{-4mm}
\end{table}

==> tables/quant-3dgen.tex <==
\begin{table}[t]
% \vspace{-4mm}
\centering
\small
\caption{
\cm{
\textbf{Quantitative evaluation of image-conditioned 3D generation.} Here, quality of both 2D rendering and 3D shapes is evaluated. As shown below, the proposed method demonstrates strong performance across all metrics. Although multi-view images-to-3D approaches like LGM achieves better performance on the FID/KID metrics, they fall short on more advanced image quality assessment metrics such as CLIP-I, MUSIQ, and performs significantly worse in 3D shape quality. For multi-view to 3D methods, we also include the number of input views (V=$\#$).
}}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Method&CLIP-I$\uparrow$&FID$\downarrow$&KID(\%)$\downarrow$&MUSIQ$\uparrow$&P-FID$\downarrow$ & P-KID(\%)$\downarrow$ &COV(\%)$\uparrow$&MMD(\textperthousand)$\downarrow$   \\
\toprule
OpenLRM                        & 86.37 & 38.41  & 1.87  & 45.46 & 35.74 & 12.60  & 39.33 & 29.08 \\
Splatter-Image                   & 84.10 & 48.80  & 3.65  & 30.33 & \cellcolor{orange}19.72 & \cellcolor{orange}7.03  & 37.66 & {30.69} \\
\midrule
One-2-3-45 (V=12)                     & 80.72 & 88.39  & 6.34 & \cellcolor{yellow}59.02 & 72.40 & 30.83  & 33.33 & 35.09 \\
CRM (V=6)                           & 85.76 & 45.53  & 1.93  & \cellcolor{orange}{64.10} & 35.21 & 13.19  & 38.83 & 28.91 \\
Lara (V=4)                          & 84.64 & 43.74  & 1.95  & 39.37 & 32.37 & 12.44  & 39.33 & 28.84 \\
LGM (V=4)        & \cellcolor{orange}{87.99} & \cellcolor{tablered}{19.93}  & \cellcolor{tablered}{0.55}  & 54.78 & 40.17 & 19.45  & 50.83 & 22.06 \\
\midrule
Shape-E                        & 77.05 & 138.53 & 11.95 & 31.51 & \cellcolor{yellow}20.98 & \cellcolor{yellow}7.41  & \cellcolor{tablered}{61.33} & \cellcolor{orange}19.17 \\
LN3Diff & \cellcolor{yellow}{87.24} & \cellcolor{yellow}29.08  & \cellcolor{yellow}0.89  & 50.39 & 27.17 & 10.02  & \cellcolor{yellow}55.17 & \cellcolor{yellow}19.94 \\
% \midrule
\textbf{Ours}         & \cellcolor{tablered}{89.06} & \cellcolor{orange}{24.21}  & \cellcolor{orange}{0.76}  & \cellcolor{tablered}{65.17} & \cellcolor{tablered}{8.72}  & \cellcolor{tablered}{3.22}  & \cellcolor{orange}{59.50} & \cellcolor{tablered}{15.48} \\
\bottomrule
\end{tabular}
}
% \end{adjustbox}
\label{tab:3d-quant-metrics}
\vspace{-3mm}
\end{table}


==> tables/shapenet.tex <==
\begin{table*}[t]
    \centering
    % \vspace{-10pt}
    % \small
    \caption{\textbf{Quantitative Comparison of Unconditional Generation on ShapeNet}. The proposed \nickname{} shows satisfactory performance on single-category generation.
    % \yslan{add latency} 
    % \cavan{table caption at the top. Use the same number of decimal points}
    }
    % \vspace{-2mm}
    \begin{tabular}{lccccc}
        \toprule
        Category&Method&FID@50K$\downarrow$&KID@50K(\%)$\downarrow$&COV(\%)$\uparrow$&MMD(\textperthousand)$\downarrow$   \\
        \midrule
        \multirow{5}*{Car}&EG3D~\cite{Chan2021EG3D}&33.33&1.4&35.32& 3.95  \\
        % \midrule
        % EG3D&--&--&--&--   \\
        &GET3D~\cite{gao2022get3d} &41.41&1.8&37.78&3.87  \\
        
        &DiffRF~\cite{muller2023diffrf}&75.09&5.1&29.01&4.52   \\
        &RenderDiffusion~\cite{anciukevivcius2023renderdiffusion}&46.5&4.1&-&-   \\
        &${\text{SSDNeRF}_\text{V=3}}$~\cite{ssdnerf}&47.72&2.8&37.84&3.46   \\
        &${\text{SSDNeRF}_\text{V=50}^{*}}$~\cite{ssdnerf}&45.37&2.1&\textbf{67.82}&2.50   \\
        % &${\text{SSDNeRF}_\text{v=3}}$~\cite{ssdnerf}&19.04&8.28&-&-   \\
        % &NFD w/ texture~\cite{Shue20223DNF}&106.06&5.5&39.21&3.85  \\
        %DiffTF &45.31&0.021&--&--   \\
        %\midrule
        &\nickname{}\textbf{(Ours)} &\textbf{17.6}&\textbf{0.49}&{43.12}& \textbf{2.32}  \\
        \midrule
        \multirow{5}*{Plane}&EG3D~\cite{Chan2021EG3D}&14.47&0.54&18.12&4.50   \\
        % \midrule
        % EG3D&--&--&--&--   \\
        &GET3D~\cite{gao2022get3d} &26.80&1.7&21.30&4.06  \\
        &DiffRF~\cite{muller2023diffrf}&101.79&6.5&37.57&3.99   \\
        % &NFD w/ texture~\cite{Shue20223DNF}&126.61&6.3&34.06&2.92   \\
        &RenderDiffusion~\cite{anciukevivcius2023renderdiffusion}&43.5&5.9&-&-   \\
        &${\text{SSDNeRF}_\text{V=3}}$~\cite{ssdnerf}&21.01&1.0&42.50&2.94   \\
        
        %DiffTF &45.31&0.021&--&--   \\
        %\midrule
        &\nickname{}\textbf{(Ours)} &\textbf{8.84}&\textbf{0.36}&\textbf{43.40}&\textbf{2.71}  \\
        \midrule
        
        \multirow{5}*{Chair}&EG3D~\cite{Chan2021EG3D}&26.09&1.1&19.17&10.31   \\
        % \midrule
        % EG3D&--&--&--&--   \\
        &GET3D~\cite{gao2022get3d} &35.33&1.5&28.07& 9.10  \\
        &DiffRF~\cite{muller2023diffrf}&99.37&4.9&17.05&14.97   \\
        % &NFD w/ texture~\cite{Shue20223DNF}&87.35&2.9&31.98&7.12   \\
        &RenderDiffusion~\cite{anciukevivcius2023renderdiffusion}&53.3&6.4&-&-   \\
        &${\text{SSDNeRF}_\text{V=3}}$~\cite{ssdnerf}&65.04&3.0&\textbf{47.54}&6.71   \\
        
        %\midrule
        %DiffTF &45.31&0.021&--&--   \\
        &\nickname{}\textbf{(Ours)} &\textbf{16.9}&\textbf{0.47}&{47.1}&\textbf{5.28}  \\
        \bottomrule
    \end{tabular}
    \label{tab:shapenet}%
    % \vspace{-2mm}
\end{table*}%

==> tables/t23d-clip.tex <==
\begin{wraptable}{r}{0.37\linewidth}
\vspace{31.0mm}
\caption{
\textbf{Quantitative Evaluation on Text-to-3D.} The proposed method outperforms existing methods on CLIP scores over two different backbones.
}
\vspace{2mm}
\label{tab:t23d-clipscore}
% \resizebox{1\linewidth}{!}{
% \vspace{2mm}
\begin{tabular}{lcc}
\toprule
Method & ViT-B/32 & ViT-L/14\\
\midrule
Point-E & 26.35 & 21.40 \\
Shape-E & 27.84 & 25.84 \\
LN3Diff & {29.12} & {27.80} \\
3DTopia & 30.10 & 28.11 \\
\midrule
Ours & \textbf{31.80} & \textbf{29.38} \\
\bottomrule
\end{tabular}
% }
\vspace{-16mm}
\end{wraptable} 
